Failure Analysis of Hadoop Schedulers using an Integration of Model Checking and Simulation

The Hadoop scheduler is a centerpiece of Hadoop, the leading processing framework for data-intensive applications in the cloud. Given the impact of failures on the performance of applications running on Hadoop, testing and verifying the performance of the Hadoop scheduler is critical. Existing approaches such as performance simulation and analytical modeling are inadequate because they are not able to ascertain a complete verification of a Hadoop scheduler. This is due to the wide range of constraints and aspects involved in Hadoop. In this paper, we propose a novel methodology that integrates and combines simulation and model checking techniques to perform a formal verification of Hadoop schedulers, focusing on the following properties: schedulability, fairness and resources-deadlock freeness. We use the CSP language to formally describe a Hadoop scheduler, and the PAT model checker to verify its properties. Next, we use the proposed formal model to analyze the scheduler of OpenCloud, a Hadoop-based cluster that simulates the Hadoop load, in order to illustrate the usability and benefits of our work. Results show that our proposed methodology can help identify several tasks failures (up to 78%) early on, i.e., before the tasks are executed on the cluster.

==> eptcsdata.tex <==
\providecommand{\firstpage}{114}
\providecommand{\publicationstatus}{T. Kutsia (Ed.): Symbolic Computation \\
in Software Science (SCSS'21)
\\
EPTCS 342, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.342.10}{10.4204/EPTCS.342.10}}
\pdfoutput=1

